Machine learning-assisted virtual patching of web applications

Web applications are permanently being exposed to attacks that exploit their vulnerabilities. In this work we investigate the application of machine learning techniques to leverage Web Application Firewall (WAF), a technology that is used to detect and prevent attacks. We propose a combined approach of machine learning models, based on one-class classification and n-gram analysis, to enhance the detection and accuracy capabilities of MODSECURITY, an open source and widely used WAF. The results are promising and outperform MODSECURITY when configured with the OWASP Core Rule Set, the baseline configuration setting of a widely deployed, rule-based WAF technology. The proposed solution, combining both approaches, allow us to deploy a WAF when no training data for the application is available (using one-class classification), and an improved one using n-grams when training data is available.

==> backgrw.tex <==
% !TEX root = main-arxiv-18.tex
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-arxiv-18"
%%% End:

\section{Web application attacks}
\label{section:WebApplicationAttacks}

Many attack taxonomies have been proposed for web application attacks \cite{}. The kind of attacks we are targeting are those related to malformed inputs, such as code injection, XSS, unauthorized directory traversal, etc. We do not consider in this work the detection of more complex attacks which spread along several \HTTP requests or requiring to consider the user session with the server.

Code injection (and in particular SQL injection) will be taken as the canonical case for ilustrating this kind of attacks. In a typical use case, the web application user is invited to fill a form with data, which the application uses internally to assemble some kind of query. In many programming languages, the programmer assembles this query by concatenating strings, which includes the data supplied by the user in the form. If such data is not correctly sanitized, an attacker may use the form fields to make the application to execute a carefully crafted piece of code that discloses unauthorized information or internally damages the application. For example, let us assume that the application displays the form field \textit{name} and assembles the following \SQL query \textit{query := \enquote{\textsc{select} * \textsc{from} users \textsc{where} name = '} + name \textsc{+} \enquote{'} }, where \textsc{+} stands for string concatenation. If the value \enquote{Juan Perez} is supplied as user name, then Juan Perez's record in the database is returned and displayed. However, should the attacker supply the string \textit{John Smith' \textsc{or} 'a'\textsc{=}'a}, the assembled query becomes \textit{\enquote{\textsc{select} * \textsc{from} users \textsc{where} name = ‘John Smith’ \textsc{or} 'a' \textsc{=} 'a'}}, which returns the records of all users. The attacker may event use more subtle payloads, in order to minimize the number of unexpected symbols in for a field intended to be a name, like for example the payload \textit{John Smith' \textsc{or nor like} 'xx}, which returns John Smith's record plus all the records of users whose name does not match the string \textit{xxx} (which, very likely, are all the users in the database). 

%However, should the attacker supply the string \textit{John Smith' \textsc{or nor like} 'xx}, the assembled query becomes \textit{\enquote{\textsc{select} * \textsc{from} users \textsc{where} name = ‘John Smith’ \textsc{or} name \textsc{not like} 'xxx'}}, which returns John Smith's record plus all the records of users whose name does not match the string \textit{xxx} (which, very likely, are all the users in the database). 

In its most general version, code injection consists in the malicious provision of unexpected input data, with the objective of modifying the intended purpose of a piece of code inside the web application. Beyond \SQL injection, this technique may be applied to any query language used by the web application, such as \textsc{xldap}, \textsc{os} commands, \textsc{xpath}, \textsc{xml} parsers, \textsc{smtp} headers, \textsc{nosql}, among others. The target of the attacker may be also the fields in the header of the \HTTP, and which are used on the web server side to perform queries about supported features, best rendering, etc. 

%From a language perspective, code injection attacks always involve mixing up two languages: the expected language for a given field and a query programming language. In the former example, the expected language for the field corresponds to personal names in English, while the query programming language is \SQL. Starting from this fact, the detection of code injection may be considered as a particular case of detecting multiple languages in a given piece of text. 



==> discussion.tex <==
% !TEX root = main-arxiv-18.tex
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-arxiv-18"
%%% End:

\section{Discussion}
\label{section:discussion}
% intro 

There exist in the literature several previous works related with the application of machine learning techniques to detect malformed input attacks. In this section we settle the main design choices that guided our approach and how they relate with them.

\textbf{Focusing on network interfaces.} Successfull attacks result from exploiting some vulnerability in the web application, like the ones listed in \cite{owasp-top-10}. Searching the application's code for such vulnerabilities and fixing them is a time consuming activity. It also requires the vulnerable application to remain off-line until the bug has been fixed, something that is not possible for critical applications. Moreover, it may be the case that its source code is not accessible or not longer available to the organization deploying the application, or cannot be patched by the organization itself. For tall these reasons we are intereseted in \textit{virtual patching}, a technique in which a second software component, external to the web application, is placed between the web application and its users. This component, usually called a Web Application Firewall (\WAF), intercepts and inspects all the \HTTP traffic between the server and the browsers, searching for attacks inside the packets' contents. Virtual patching may be applied to any web application and relays on standardized and public protocols, such as \HTTP.  Other alternative approaches such as \cite{BockermannAM09}, \cite{KarPS161}, \cite{KarPS162} rather focus on the database tiers and database firewalls (\DBF). Those works also apply anomally detection techniques, but to the flow of SQL sentences from the application server to its database server. We prefer to focus on the \WAF approach rather than on the \DBF one for three reasons. First, in \DBF the scope is restricted to detect only SQL injection attacks. On the contrary, a \WAF is able to intercept a broaderer class of attacks, including \XSS, any form of code injection, path traversal, etc. Second, the protocol used for connecting to the database is usually propietary and depends on each database, so the \DBF approach does not provide the interoperability we are looking for. Finally, the \DBF approach eventually lays on the internal interfaces of the web application, so a change in the application implementation could require re-training the anomally detection component in the \DBF. To enforce protection interoperability across application changes, we prefer to focus on the analysis of the external bounderies of the web application, that is, on the \HTTP traffic.

\textbf{Focusing on the application layer.} One of the seminal works in anomally detection techniques was developped by Wang and Stolfo. In \cite{wang2004anomalous}, where they introduced PAYL, a payload-based anomaly detector for intrusion detection. Their approach consists in comparing the byte frequency distribution in network packets using (a simplified) Mahalanobis distance. Accordingly with the current attack vectors of that time, their objective was not focused on protecting an internal network from packats carrying worms or other forms of malware. Consistently, their model works on TPC packets, that is, on the network OSI layer. As the byte distribution heavily depends on the application protocol, they divide the stream into smaller groups of packets, grouping them by destination port and by payload length. They applied PAYL to the traffic to port 80 (\HTTP) of the 1991 \textsc{darpa ids} dataset, obtaining excellent detection results. However, such impressive results relate to the attack vectors of 1999. Indeed, the \textsc{darpa ids 99} dataset did not contain not contain any of the \textsc{owasp top 10} attacks \cite{DARPAIDSDataset-attacks}\footnote{This is not suprising, as web applications arose during the 2000, and SQL injection was first reported in December 1998 \cite{forristal1998}}. As a consequence, while Wang and Stolfo reports in \cite{wang2004anomalous} on a 100\% detection rate for traffic on port 80 of the \textsc{darpa ids} dataset based on byte frequency distribution of the uparsed \TCP payloads, performing the same analysis on the \textsc{cisc2010} dataset yielded a detection rate of only 40\% of the true anomalous cases. This low performance has been also independently reported by Ingham and Inoue in \cite{IngramInoue}. The reason is that token distribution does vary from one \HTTP field or web application parameter to another, which are spread along several \TCP packets. Protecting web applications require shifting the analysis to the application OSI layer, focusing on \HTTP requests. 
TOD: dar datos mas precisos de cuantos ataques en Wang y Stolfo. Citar quienes se focalizan en application layer.

\textbf{\textsc{http} request structure.} Among the works foucusing on the application layer, a few of them consider each \HTTP request as a single unstructured document to be analyzed and classified \cite{gallagher2009classification,ecml-pkdd-challenge}. This technique preveals when the approach is focused on attack signature identification and classification. Anomaly detection approaches usually perform some partial parsing of the \HTTP structure, for example in \cite{EstevezTapiador2004175,kruegel2003anomaly}. In those works, the parsing is reduced to the structure of the \URI, splitting the URL from the web application parameters. In our proposal we go further, splitting the request contents into the contents of its header, header fields, and web application parameters (either appendend to the \URI or in the \HTTP body)\footnote{In the sequel, we use the generic term \textit{field} to refer to any of these sub-parts into which the \HTTP request is divided.}. We advocate for this approach for several resasons. First, all fields are subject to attacks, as illustrated in the \PKDD dataset \cite{pkddsummary}. Therefore, there is no reason to restrict the analysis to the \URI. Also, each field has its own independent language, which may be quite different from the language of other fields. This is confirmed by the experiments made by Ingrham and Inoue in \cite{IngramInoue} on the parameters of the URI. As a consecuence, a much more specific and biased contents can be extracted from each one than from the whole request. In \cite{kruegel2003anomaly}, Kruegel and Vigna propose to take advantage of the web parameter names themselves and the order in which they are presented. In our approach the field names are only exploited to select the language to be used for a specific piece of contents inside the \HTTP request. The only attribute drawn from the field names themselves is whether they were met during the training. This is because several attacks attempt to exploit well-known buggous PHP scripts that could be present in the server, which they try to execute assigning some crafter values for their parameters. These parameters have usually nothing to do with the regular parameters of the web application, so their presence is a good indicator for this kind of attacks. Beyond this attribute, we do not collect any other relevant statistical information from the field names themselves. 

\textbf{Tokens as features.} The contents of each request field is a string, so most of the anomaly detection approaches make use of document classification, \NLP and information retrieval techniques. The attributes extracted from the request are either the number of ocurrences of a given set of \textit{tokens} into which the string is divided, or their frequency relative to the field contents length. As content languages may significantly vary from one field to another, in most of the previous work tokens are just n-grams 
\cite{wang2004anomalous,wang2006anagram,kruegel2003anomaly,torrano2010anomaly,Corona08,CoronaAG09,closeLookToNgrams}. An n-gram is a sequence of characters. These characters are usually consecutive, even though \cite{Corona08} shows that using $n$ characters which are $m$ positions aways one from the other may also be an alternative. N-grams provide an attractive tool, as they can be easily drawn from the contents in linear time, just shifting a slice window all along the string. Moreover, this approach does not require any previous knowledge about the structure of the field contents nor the grammar for generating them. However, the n-gram frequency approach may not be the most relevant attribute in some particular cases. Consider for instance the case of the 
\URI: in the contents %\url{https://www.example.com/test}
 what is unexpected is the ocurrence of the subdirectory \texttt{test}, rather that the frequency of the letter 
\texttt{t} in the whole \URI. Moreover, in this case exists a clear delimiter character (the slash) which enables to divide the contents into tokens, namely, the words of the directory ressources. In our work, we generalize and extend the idea of n-grams and words in the following way: the contents string is first split into a sequence of sub-strings (tokens) separated by other sub-strings meeting a regular expression (the \textsl{delimiters}). Then, we consider n-grams formed with sequences of these tokens. The traditional n-gram analysis is a particular case of this general scheme, where the delimiter is the empty sequence and the tokens are characters. In the case of an URI, the delimiter is the slash character. Other fields, such as \texttt{Accept-Encoding} or \texttt{Accept-Language} also make use of commas and semicolonns as delimiters, and can be addressed in terms of words instead of characters.

\textbf{Higher order n-grams.} Initial attempts for using n-gram analysis on \HTTP requests focused on monograms and single character distributions \cite{wang2004anomalous,torrano2010anomaly}. However, Kolesnikov and Lee \cite{Kolesnikov04advancedpolymorphic} and  Pastrana et al. \cite{Pastrana2015} have shown that short n-grams are vulnerable to mimicry attacks, in which the attacker carefully adds characters in order to get closer to the n-gram distribution expected by the \WAF. Mimicry attacks become much more challenging when using higher n-grams \cite{wang2006anagram}. Opposite to \cite{}, we do not use n-grams of a fixed length $n$, but all the n-grams of any length up to a given model parameter $n$ that can be adjusted for each case. As we will show, when the structure of the \HTTP requests is exploited, a bound of $n$=3 is enough for obtaining a high rate of detection with acceptable false positive rate. This contrast with the results in \cite{}, where much longer n-grams are required for reaching a similar detection rate.

\textbf{Token abstraction.} In practice, not all tokens are actually relevant. For example, the \IP address 168.192.0.1 does not better characterise valid requests than the IP 168.192.0.2. On the other side, counting the number of ocurrences of each particular \IP address is more prone to overfitting. A similar situation arises with the \URI: as many applications generate parts of the \URI dynamically, it is useless to count the random numbers ocurring in those \URI. For this reason, several authors do not directly work on the tokens themselves, but rather on some simplification of them. In \cite{CoronaAG09}, Corona et al. abstracts away numbers and alphanumeric sequences, representing each category with a single symbol. In \cite{torrano2010anomaly}, Torrano, Perez and Mara\~n\'on only consider the frequencies of three sets of symbols: characters, numbers and special symbols, as well as the list of special symbols used in each field. In general, what is counted is the number of symbols after applying some forget functor on the set of tokens, which abstracts aways irrelevant differences. In our experiments, this functor performs the following transformations: (a) letters are uncapitalized, (b) accents are removed (for instance, the letter \textit{\'a} is transformed into \textit{a}) and (c) n-grams made only of numbers are collapsed into the capital letter \enquote{\textit{N}}. Removing information simplifies and speeds up the analysis. However, if too much information is removed from the tokens some attacks may become indistinguishible from correct behavior, so an adecuate compromise shall be found.

\textbf{Complementary approaches.} The problem of protecting a web application can be analyzed using two different machine learning approaches: as an \textit{anomally detection} problem, and as a \textit{classification} problem. The first approach focuses on characterizing which are the expected (valid) input values for the web application, and considers any anomalous input supplied to the application as a potential attack from the user. Protecting the application therefore amounts to outiler detection from a training dataset of valid inputs, and therefore relates to unsupervised machine learning. The second approach consists in starting from a collection of inputs, each one labelled either as a valid input, or as some kind of attack from an attack taxonomy. In this approach, protecting the web application amounts to classify a new given input from a previous training phase based on supervised learning. Most of previous work relays on anomally detection \cite{}, as it has several advantages. First, as it consider as problematic any behavoir different from the usual one, it can potentially detect 0-days attacks. Also, training the \WAF only requires a collection of \HTTP requests produced by friendly users, getting rid of the task of labelling the \HTTP requests. However, as already noticed in \cite{closeLookToNgrams}, this approach cannot provide an answer to all possible attack scenarios. This is because some of the web application input data may be random data by its very nature. Consider for instance a web application parameter carrying a user password. It can be made of any combination of symbols, and in principle all combination should be equally likely. In such cases there is no hope to find a strong language signature for the field, nor to reject a chosen password on the basis that it is not frequently used. Furthermore, for security reasons, it would not be advisable for the \WAF to store information about the distribution of such sensible parameters. In those cases, where there is no a priori expected behavior, it is necessary to adopt a symmetric approach, and search for attack signatures inteh field according to the current state of the art. This amounts to say searching for carefully selected tokens, extracted from a labelled training dataset and representing the knowledge of the security expert on the current attack vectors. This technique, that we call \textit{normality detection} approach, deems the \HTTP request as valid by default when it cannot be recognized as an attack according to the previous training. \egnote{Rodrigo, Alvaro, Gustavo: complete the main properties of your approach please}.

\textbf{Normality detection.} \egnote{Explain the one-class approach, relation to previous work.}


To summarize, our approach consists in focusing the analysis in the application layer, more precisely in the \HTTP interfaces. It takes advantage of the internal structure of the \HTTP requests, extracting features from the text contained in all the \HTTP fields after aplying some forgetful functor on such text. From this basis, two complementary approaches are combined: anomaly detection with respect to the expected language signture of each field using high-order n-grams up to some $n$, and normality detection based on \egnote{COMPLETE:such and such property} to tackle those fields which have no a priori biased distribution \egnote{or as a confirmation on those fields which are classified as anomalous????}.
